A Library for Constraint Consistent Learning

This paper introduces the first, open source software library for Constraint Consistent Learning (CCL). It implements a family of data-driven methods that are capable of (i) learning state-independent and -dependent constraints, (ii) decomposing the behaviour of redundant systems into task- and null-space parts, and (iii) uncovering the underlying null space control policy. It is a tool to analyse and decompose many everyday tasks, such as wiping, reaching and drawing. The library also includes several tutorials that demonstrate its use with both simulated and real world data in a systematic way. This paper documents the implementation of the library, tutorials and associated helper methods. The software is made freely available to the community, to enable code reuse and allow users to gain in-depth experience in statistical learning in this area.

==> ext/tex/abbreviations.tex <==
% define \gnewcommand and \grenewcommand for global specification of commands (used for \newabbreviation command)
\usepackage{etoolbox}
\makeatletter
\def\gnewcommand{\g@star@or@long\gnew@command}
\def\grenewcommand{\g@star@or@long\grenew@command}
\def\g@star@or@long#1{% 
  \@ifstar{\let\l@ngrel@x\global#1}{\def\l@ngrel@x{\long\global}#1}}
\def\gnew@command#1{\@testopt{\@gnewcommand#1}0}
\def\@gnewcommand#1[#2]{%
  \kernel@ifnextchar [{\@gxargdef#1[#2]}%
                {\@argdef#1[#2]}}
\let\@gxargdef\@xargdef
\patchcmd{\@gxargdef}{\def}{\gdef}{}{}
\let\grenew@command\renew@command
\patchcmd{\grenew@command}{\new@command}{\gnew@command}{}{}
\makeatother
% define newabbreviation command
\newcommand{\newabbreviation}[2]{#1\ (\grenewcommand{#1}{#2\xspace}#1)}

% months
\newcommand{\jan      }{January}
\newcommand{\feb      }{February}
\newcommand{\mar      }{March}
\newcommand{\apr      }{April}
\newcommand{\may      }{May}
\newcommand{\jun      }{June}
\newcommand{\jul      }{July}
\newcommand{\aug      }{August}
\newcommand{\sep      }{September}
\newcommand{\oct      }{October}
\newcommand{\nov      }{November}
\newcommand{\dec      }{December}

% King's
\newcommand{\KCL    }{King's College London}
\newcommand{\NMS    }{Natural and Mathematical Sciences}
\newcommand{\CORE   }{the Centre for Robotics Research}
\newcommand{\RLL    }{Robot Learning Lab}
\newcommand{\WLab   }{Wheatstone Innovation Lab}

% Universities/research institutes
\newcommand{\TUM    }{Technische Universit\"{a}t Munich}
\newcommand{\MIT    }{Massachusetts Institute of Technology}

% funding bodies/schemes
\newcommand{\ERC    }{European Research Council}
\newcommand{\EPSRC  }{Engineering and Physical Sciences Research Council}
\newcommand{\CC     }{Crafts Council}
\newcommand{\JSPS   }{Japan Society for the Promotion of Science}
\newcommand{\AHDB   }{Agriculture and Horticultural Development Board}
\newcommand{\RSSB   }{Rail Safety and Standards Board}
\newcommand{\CONACYT}{Consejo Nacional de Ciencia y Tecnologia}
\newcommand{\HZOZO  }{Horizon 2020}
\newcommand{\FPZ    }{Seventh Framework Program}
\newcommand{\KTP    }{Knowledge Transfer Partnership}
\newcommand{\RIA    }{Research and Innovation Action}
\newcommand{\CTF    }{College Teaching Fund}

% journals, conferences
\newcommand{\TRo    }{IEEE Transactions on Robotics}
\newcommand{\TNSRE  }{IEEE Transactions on Neural Systems and Rehabilitation Engineering}
\newcommand{\TMech  }{IEEE Transactions on Mechatronics}
\newcommand{\IJRR   }{International Journal of Robotics Research}
\newcommand{\NC     }{Neural Computation}
\newcommand{\AURO   }{Autonomous Robots}
\newcommand{\ICRA   }{IEEE International Conference on Robotics and Automation}
\newcommand{\IROS   }{IEEE International Conference on Intelligent Robots and Systems}
\newcommand{\RSS    }{Robotics: Science and Systems}
\newcommand{\Humanoids}{IEEE International Conference on Humanoid Robots}
\newcommand{\AIM    }{ASME/IEEE International Conference on Advanced Intelligent Mechatronics}
\newcommand{\ICORR  }{IEEE International Conference on Rehabilitation Robotics}
\newcommand{\BioRob }{IEEE International Conference on Biomedical Robotics and Biomechatronics}
\newcommand{\NIPS   }{Advances in Neural Information Processing Systems}

% people
\newcommand{\PI     }{principle investigator}
\newcommand{\CoI    }{co-investigator}
\newcommand{\PDRA   }{postdoctoral research assistant}
\newcommand{\UG     }{undergraduate}
\newcommand{\PG     }{postgraduate}
\newcommand{\TA     }{teaching assistant}
\newcommand{\MH     }{Matthew Howard}

% certificates/qualifications
\newcommand{\BSc}    {BSc}
\newcommand{\MSci}   {MSci}
\newcommand{\MSc}    {MSc}
\newcommand{\PhD}    {PhD}
\newcommand{\PGCAPHE}{Postgraduate Certificate in Academic Practice in Higher Education}

% machine learning
\newcommand{\RL     }{reinforcement learning}
\newcommand{\HMMs   }{hidden Markov models}

% robotics
\newcommand{\RAS    }{Robotics and autonomous systems}
\newcommand{\ROS    }{Robot Operating System}
\newcommand{\PbD    }{programming by demonstration}
\newcommand{\DoF    }{degrees of freedom}
\newcommand{\VIA    }{variable impedance actuator}
\newcommand{\EMG    }{electromyography}
\newcommand{\VPSA   }{variable physical stiffness actuator}
\newcommand{\CCL    }{constraint consistent learning}

% bibliographies
\newcommand{\Journal}{Journal}
\newcommand{\Eng    }{Engineering}
\newcommand{\Trans  }{Transactions}

% general
\newcommand{\WP     }{work package}
\newcommand{\TRL    }{technology readiness level}
\newcommand{\SMEs   }{small and medium enterprises}
\newcommand{\OA     }{open access}
\newcommand{\ICT    }{information and communication technology}
\newcommand{\HCI    }{human computer interfaces}



==> ext/tex/graphics.tex <==
% use graphicx for including images, set default image path
\usepackage{graphicx}
\graphicspath{{fig/}} 



==> ext/tex/meta.tex <==
\newcommand{\thetitle}         {}
\newcommand{\theshorttitle}    {}

\newcommand{\theauthor}        {Matthew Howard}
\newcommand{\theshortauthor}   {M. Howard}


==> usage.tex <==
\section*{Usage notes}~\\%[1ex]
%\paragraph*{Comments}~\\%[1ex]
\noindent Use \texttt{\textbackslash yourinitials\{your comment\}} to add comments/to dos. For example,
\underline{J}oe \underline{B}loggs adds comments using \texttt{\textbackslash jb\{Comment.\}}.\jb{These comments will appear as margin notes. They will also appear in the todo list on the first page.} \\[2ex]
\noindent Use \texttt{\textbackslash atInitials} to address your comment to someone (\eg \texttt{\textbackslash jb\{\textbackslash atMH: Please fix this.\}}).\\[2ex]
You can mark a comment as resolved using \texttt{\textbackslash done\{Comment text.\}}, (\eg \texttt{\textbackslash jb\{\textbackslash done\{\textbackslash atMH: Please fix this.\}\}}). It will then be formatted like this: \done{\atMH: Please fix this.}.\\[2ex]
\commentcolourcode\\[1ex]
%\noindent\note{Guidance text from the call is formatted like this.}\\[2ex]
%\paragraph*{Work packages/tasks/deliverables, referencing}~\\%[1ex]
%\emph{Work package descriptions} are added as:\\[1ex]
%\texttt{\textbackslash work package\{wp\_label\}\{Work package title\}\{Lead partner\}\{start\_month\}\{end\_month\}\{\\
%Objectives description text.\\
%\}\\
%\{\\
%Task descriptions.\\
%\}\\
%\{\\
%Deliverables descriptions.\\
%\}\\
%}\\[1ex]
%To refer to work packages in the text, you can use:\\[1ex]
%\texttt{\textbackslash wpref\{wp\_label\}} (will format the reference as `WPX'), or \\
%\texttt{\textbackslash ref\{wp:wp\_label\}} (will just give the WP number, \ie `X').\\[2ex]
%%
%To add \emph{task descriptions} you can use:\\[1ex]
%\texttt{\textbackslash task\{task\_label\}\{Task title\}\{List of partners (lead partner in \textbf{bold})\}\{start\_month\}\{end\_month\}\{\\
%Task description text.\}}\\[1ex]
%To refer to that task in the text, you can use:\\[1ex]
%\texttt{\textbackslash tkref\{task\_label\}} (will format the reference as `TX.X'), or \\
%\texttt{\textbackslash ref\{tk:task\_label\}} (will just give the number, \ie `X.X').\\[2ex]
%%
%To add \emph{deliverables descriptions} you can use:\\[1ex]
%\texttt{\textbackslash deliverable\{deliverable\_label\}\{Deliverable description text\}\{Partner(s) responsible\}\{month\_due\}\{deliverable\_type\}\{dissemination\_level\}}\\[1ex]
%To refer to it in the text, you can use:\\[1ex]
%\texttt{\textbackslash dref\{deliverable\_label\}} (will format the reference as `DX.X'), or \\
%\texttt{\textbackslash ref\{d:deliverable\_label\}} (will just give the number, \ie `X.X').\\[2ex]

\listoftodos~\\[2ex]
\clearpage\setcounter{page}{1}



